Reconstruction and Simulation of Elastic Objects with Spring-Mass 3D Gaussians

Reconstructing and simulating elastic objects from visual observations is crucial for applications in computer vision and robotics. Existing methods, such as 3D Gaussians, model 3D appearance and geometry, but lack the ability to estimate physical properties for objects and simulate them. The core challenge lies in integrating an expressive yet efficient physical dynamics model. We propose Spring-Gaus, a 3D physical object representation for reconstructing and simulating elastic objects from videos of the object from multiple viewpoints. In particular, we develop and integrate a 3D Spring-Mass model into 3D Gaussian kernels, enabling the reconstruction of the visual appearance, shape, and physical dynamics of the object. Our approach enables future prediction and simulation under various initial states and environmental properties. We evaluate Spring-Gaus on both synthetic and real-world datasets, demonstrating accurate reconstruction and simulation of elastic objects. Project page: https://zlicheng.com/spring_gaus/.

==> sec/3_preliminary.tex <==
\section{Preliminary}

This section introduces 3D Gaussian Splatting \cite{kerbl3Dgaussians}, the foundational method underlying our approach. Gaussian Splatting employs a set of 3D Gaussian kernels to represent a scene. These kernels are characterized by a full 3D covariance matrix $\Sigma$, defined in world space and centered at point $\boldsymbol{\mu}$:
\begin{equation}
    G(\boldsymbol{x}) = e^{-\frac{1}{2}(\boldsymbol{x})^T\Sigma^{-1}(\boldsymbol{x})},
\end{equation}
%
where $\boldsymbol{\mu}$ is the mean of the Gaussian distribution, and $\boldsymbol{x}$ is the independent variable of the Gaussian distribution.
%
The covariance matrix $\Sigma$ can be decomposed into a rotation matrix $R$ and a scaling matrix $S$, such that $\Sigma = RSS^TR^T$.

The Splatting process, designed to render Gaussian kernels into a 2D image, involves two main steps: \emph{(1)} projecting the Gaussian kernels into camera space, and \emph{(2)} rendering the projected kernels into image space. The projection process is defined as:
\begin{equation}
    \Sigma^{\prime} = JW\Sigma W^TJ^T,
\end{equation}
where $\Sigma^{\prime}$ represents the covariance matrix in camera coordinates, $W$ is the transformation matrix, and $J$ denotes the Jacobian of the affine approximation of the projective transformation. The rendered color $C$ of each pixel is computed as:
\begin{equation}
    C = \sum_{i\in N}T_i\alpha_i \boldsymbol{c_i},
    \label{eq:rendering}
\end{equation}
where $T_i$ represents the transmittance, defined as $\Pi_{j=1}^{i-1}\alpha_j$. The term $\alpha_i$ denotes the alpha value for each Gaussian, which is calculated using the expression $1-e^{-\sigma_i\delta_i}$, where \(\sigma_i\) is the opacity factor. Additionally, $\boldsymbol{c_i}$ refers to the color of the Gaussian along the ray within the interval $\delta_i$.

The learnable parameters for each Gaussian kernel include a point center $\boldsymbol{\mu}$, a 3D scaling vector $\boldsymbol{s}$, a quaternion $\boldsymbol{q}$, a color $\boldsymbol{c}$, an opacity factor $\sigma$, and a set of spherical harmonics (SH) coefficients. These SH coefficients are employed to represent the view-dependent component of the radiance field.

==> sec/exp/ablation.tex <==
\subsection{Ablation Study}

\input{sec/img/ablation.tex}

In our approach, we employ a soft vector $\eta$ to dynamically regulate both the quantity and intensity of springs linked to the anchor points. This strategy is illustrated in \cref{tab:ablation}, showcasing its effectiveness. Our method's capability to simulate using very sparse anchors allows for the individual optimization of physical parameters for each anchor point. This contrasts with PAC-NeRF, which utilizes tens of thousands of particles, making it challenging to optimize the physical parameters for each particle infeasible. Consequently, PAC-NeRF faces limitations in accurately modeling objects composed of heterogeneous materials. In contrast, our methodology is adept at handling such complexities. As depicted in \cref{fig:ablation} and \cref{tab:ablation}, we present the outcomes on a heterogeneous object that is segmented into various sections, each with distinct physical properties, thereby demonstrating our model's superior adaptability in capturing the nuanced dynamics of objects with variable material composition.

==> sec/img/spring_ground.tex <==
\begin{figure}[!h]
        \centering
        \includegraphics[width=\textwidth]{figs/spring_ground_duck.pdf}
        \caption{Removable ground, we set the ground as a spring in this demo.}
        \label{fig:removable_ground}
\end{figure}
